Thermodynamic Limits of Proof

Every irreversible recorded distinction has a positive thermodynamic work floor. Landauer's principle supplies the ideal bound $\varepsilon\ge k_B T\ln 2$ per irreversible bit, experimentally verified to $\pm 10\%$. Proof available to an agent is checkable information for that agent: some substrate must produce, retain, and expose evidence that excludes answer-changing alternatives. A finite detector array operating at temperature $T$ for finite time has finite signal-acquisition capacity. Combining finite causal access, positive retained-record cost, and exact lower bounds on required records gives the Physical Counting Impossibility Theorem: no fixed-budget substrate can provide universal exact proof once the retained-record lower bound exceeds the declared budget. The theorem requires exactly $B<\infty$ and $\varepsilon>0$. An answer reports a value; proof supplies checkable grounds for accepting it. A reversible device may compute an answer and erase its scratch history, but proof requires retained, inspectable records. A global answer register, oracle response, entanglement witness, finite survey catalog, or trusted device output supplies proof only through an interface that exposes the relevant grounds to the verifier. A proposed interface must identify the retained-record lower-bound family $R(n)$ it induces. Sound operational claims about efficient solvability inherit the same finite-budget obstruction when their acceptance would license universal exact proof. Substrate-free derivability has proof status only when a physical verification event makes it available to an agent.

==> content/assumption_ledger_auto.tex <==
% Auto-generated by scripts/build_papers.py. Do not edit manually.
% Generated: 2026-06-05T15:34:27.968755
\subsection{Assumption Ledger (Auto)}
\paragraph{Source files.}
\begin{itemize}
\item \nolinkurl{DecisionQuotient/ClaimClosure.lean}
\item \nolinkurl{DecisionQuotient/HandleAliases.lean}
\item \nolinkurl{DecisionQuotient/StochasticSequential/ClaimClosure.lean}
\item \nolinkurl{DecisionQuotient/StochasticSequential/Hierarchy.lean}
\end{itemize}
\paragraph{Assumption bundles and fields.}
\begin{itemize}
\item (No assumption bundles parsed.)
\end{itemize}
\paragraph{Conditional closure handles.}
\begin{itemize}
\item \nolinkurl{DQ.anchor_sigma2p_complete_conditional}
\item \nolinkurl{DQ.cost_asymmetry_eth_conditional}
\item \nolinkurl{DQ.dichotomy_conditional}
\item \nolinkurl{DQ.minsuff_collapse_to_conp_conditional}
\item \nolinkurl{DQ.minsuff_conp_complete_conditional}
\item \nolinkurl{DQ.sufficiency_conp_complete_conditional}
\item \nolinkurl{DQ.tractable_subcases_conditional}
\end{itemize}
\paragraph{First-principles Bayes derivation handles.}
\begin{itemize}
\item \nolinkurl{DQ.BayesOptimalityProof.KL_eq_sum_klFun}
\item \nolinkurl{DQ.BayesOptimalityProof.KL_eq_zero_iff_eq}
\item \nolinkurl{DQ.BayesOptimalityProof.KL_nonneg}
\item \nolinkurl{DQ.BayesOptimalityProof.bayes_is_optimal}
\item \nolinkurl{DQ.BayesOptimalityProof.crossEntropy_eq_entropy_add_KL}
\item \nolinkurl{DQ.BayesOptimalityProof.entropy_le_crossEntropy}
\item \nolinkurl{DQ.Foundations.bayes_from_conditional}
\item \nolinkurl{DQ.Foundations.complete_chain}
\item \nolinkurl{DQ.Foundations.counting_additive}
\item \nolinkurl{DQ.Foundations.counting_nonneg}
\item \nolinkurl{DQ.Foundations.counting_total}
\item \nolinkurl{DQ.Foundations.dq_equivalence}
\item \nolinkurl{DQ.Foundations.dq_in_unit_interval}
\item \nolinkurl{DQ.Foundations.dq_one_iff_perfect_info}
\item \nolinkurl{DQ.Foundations.dq_zero_iff_no_info}
\item \nolinkurl{DQ.Foundations.entropy_contraction}
\item \nolinkurl{DQ.Foundations.mutual_info_nonneg}
\item \nolinkurl{DQ.bayesian_dq_matches_physics_dq}
\item \nolinkurl{DQ.chain_rule}
\item \nolinkurl{DQ.dq_derived_from_bayes}
\item \nolinkurl{DQ.dq_is_bayesian_certainty_fraction}
\end{itemize}
\paragraph{Compact Bayes handle IDs.}
\begin{itemize}
\item \nolinkurl{FN7} $\to$ \nolinkurl{DQ.BayesOptimalityProof.KL_nonneg}
\item \nolinkurl{FN8} $\to$ \nolinkurl{DQ.BayesOptimalityProof.entropy_le_crossEntropy}
\item \nolinkurl{FN12} $\to$ \nolinkurl{DQ.BayesOptimalityProof.crossEntropy_eq_entropy_add_KL}
\item \nolinkurl{FN14} $\to$ \nolinkurl{DQ.BayesOptimalityProof.bayes_is_optimal}
\item \nolinkurl{FN15} $\to$ \nolinkurl{DQ.BayesOptimalityProof.KL_eq_sum_klFun}
\item \nolinkurl{FN16} $\to$ \nolinkurl{DQ.BayesOptimalityProof.KL_eq_zero_iff_eq}
\item \nolinkurl{BB1} $\to$ \nolinkurl{DQ.BayesianDQ}
\item \nolinkurl{BB2} $\to$ \nolinkurl{DQ.BayesianDQ.certaintyGain}
\item \nolinkurl{BB3} $\to$ \nolinkurl{DQ.dq_is_bayesian_certainty_fraction}
\item \nolinkurl{BB4} $\to$ \nolinkurl{DQ.bayesian_dq_matches_physics_dq}
\item \nolinkurl{BB5} $\to$ \nolinkurl{DQ.dq_derived_from_bayes}
\item \nolinkurl{BF1} $\to$ \nolinkurl{DQ.certainty_of_not_nondegenerateBelief}
\item \nolinkurl{BF2} $\to$ \nolinkurl{DQ.nondegenerateBelief_of_uncertaintyForced}
\item \nolinkurl{BF3} $\to$ \nolinkurl{DQ.forced_action_under_uncertainty}
\item \nolinkurl{BF4} $\to$ \nolinkurl{DQ.bayes_update_exists_of_nondegenerateBelief}
\end{itemize}


==> content/proof_hardness_index_auto.tex <==
% Auto-generated by scripts/build_papers.py. Do not edit manually.
% Generated: 2026-06-05T15:34:28.870243
% Manuscript: paper4_toc
\begingroup
\scriptsize
\sloppy
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.12}
\begin{longtable}{@{}>{\raggedright\arraybackslash}m{0.19\linewidth}>{\raggedright\arraybackslash}m{0.13\linewidth}>{\raggedright\arraybackslash}m{0.26\linewidth}>{\raggedright\arraybackslash}m{0.38\linewidth}@{}}
\toprule
\textbf{Manuscript handle} & \textbf{Hardness profile} & \textbf{Regime tags} & \textbf{Lean support} \\
\midrule
\endfirsthead
\toprule
\textbf{Manuscript handle} & \textbf{Hardness profile} & \textbf{Regime tags} & \textbf{Lean support} \\
\midrule
\endhead
\endfoot
\bottomrule
\endlastfoot
\nolinkurl{cor:finite-budget-threshold-impossibility} & \nolinkurl{unspecified} & - & \LH{PBC18} \\
\midrule
\nolinkurl{cor:operational-provability} & \nolinkurl{unspecified} & - & \LH{CI17}, \LH{CI18}, \LH{CI19}, \LH{CI20}, \LH{CI21}, \LH{CI22}, \LH{CI23}, \LH{CI24}, \LH{CI25}, \LH{CI26}, \LH{PH26}, \LH{PROV2}, \LH{PROV3}, \LH{PROV5}, \LH{PROV7}, \LH{PROV8}, \LH{PROV9}, \LH{PROV10}, \LH{PROV11}, \LH{PROV12}, \LH{PROV13}, \LH{PROV14}, \LH{PROV15}, \LH{PROV16}, \LH{PROV17}, \LH{PROV18}, \LH{PROV19}, \LH{PROV20}, \LH{PROV21}, \LH{PROV22}, \LH{PROV23}, \LH{PROV24}, \LH{PROV25}, \LH{PROV26}, \LH{PROV27}, \LH{PROV28}, \LH{PROV29}, \LH{PROV30}, \LH{PROV31}, \LH{PROV32}, \LH{PROV33}, \LH{PROV34}, \LH{PROV35}, \LH{PROV36}, \LH{PROV37}, \LH{PROV38}, \LH{PROV39}, \LH{PROV40} \\
\midrule
\nolinkurl{prop:finite-budget-necessity-countermodels} & \nolinkurl{unspecified} & - & \LH{PH31}, \LH{PH32}, \LH{PH33} \\
\midrule
\nolinkurl{prop:mh-ctc-bridge-boundary} & \nolinkurl{unspecified} & - & \LH{GI13}, \LH{GI14}, \LH{GI15}, \LH{GI16} \\
\midrule
\nolinkurl{prop:physical-oracle-trust-budget} & \nolinkurl{unspecified} & - & \LH{PROV66}, \LH{PROV67}, \LH{PROV68}, \LH{PROV69}, \LH{PROV70}, \LH{PROV71}, \LH{PROV72}, \LH{PROV73} \\
\midrule
\nolinkurl{prop:tokenhood-insufficient-certifier-extraction} & \nolinkurl{unspecified} & - & \LH{PROV31}, \LH{PROV36}, \LH{PROV58}, \LH{PROV59}, \LH{PROV60}, \LH{PROV61}, \LH{PROV62} \\
\midrule
\nolinkurl{thm:physical-impossibility-universal-exact} & \nolinkurl{unspecified} & - & \LH{PH11}, \LH{PH12}, \LH{PH13}, \LH{PH14}, \LH{PH15}, \LH{PH26}, \LH{PH27} \\
\midrule
\nolinkurl{thm:query-physical} & \nolinkurl{unspecified} & - & \LH{CI3}, \LH{CI4}, \LH{CI5}, \LH{CI6} \\
\midrule
\nolinkurl{thm:resolution-sufficient} & \nolinkurl{unspecified} & - & \LH{CI3}, \LH{CI4}, \LH{CI5}, \LH{CI6}, \LH{CI27}, \LH{CI28}, \LH{CI29} \\
\midrule
\nolinkurl{thm:thermo-derived} & \nolinkurl{unspecified} & - & \LH{BA9}, \LH{CI5}, \LH{CI6}, \LH{CI7} \\
\bottomrule
\end{longtable}
\endgroup

\noindent\textit{Auto summary: indexed 10 claims by hardness profile (unspecified=10).}


==> lean-handle-macros.tex <==
% Auto-generated by scripts/build_papers.py. Do not edit manually.
% Lean handle macro definitions: compact footnote markers in body text
\providecommand{\LH}[1]{}
\renewcommand{\LH}[1]{\leavevmode\nobreak\hyperlink{lh:#1}{\mbox{\ttfamily\nolinkurl{#1}}}}
\providecommand{\LHrng}[3]{}
\renewcommand{\LHrng}[3]{\leavevmode\nobreak\hyperlink{lh:#1#2}{\mbox{\ttfamily\nolinkurl{#1#2-#3}}}}
\newif\ifleanmetaseen
\leanmetaseenfalse
\makeatletter
\providecommand{\leanmetapendinghandles}{}
\global\let\leanmetapendinghandles\@empty
\providecommand{\leanmetapending}[1]{}
\renewcommand{\leanmetapending}[1]{\def\leanmetatest{#1}\ifx\leanmetatest\@empty\global\let\leanmetapendinghandles\@empty\else\gdef\leanmetapendinghandles{#1}\fi}
\providecommand{\leanmetaproofpendinghandles}{}
\global\let\leanmetaproofpendinghandles\@empty
\providecommand{\leanmetaproofpending}[1]{}
\renewcommand{\leanmetaproofpending}[1]{\def\leanmetatest{#1}\ifx\leanmetatest\@empty\global\let\leanmetaproofpendinghandles\@empty\else\gdef\leanmetaproofpendinghandles{#1}\fi}
\providecommand{\leanmetaheadmark}{}
\renewcommand{\leanmetaheadmark}{\ifx\leanmetapendinghandles\@empty\else\refstepcounter{footnote}\footnotemark[\value{footnote}]\footnotetext[\value{footnote}]{\ifleanmetaseen\else Lean: \global\leanmetaseentrue\fi\leanmetapendinghandles}\global\let\leanmetapendinghandles\@empty\fi}
\providecommand{\leanmetaproofmark}{}
\renewcommand{\leanmetaproofmark}{\ifx\leanmetaproofpendinghandles\@empty\else\ifhmode\unskip\footnote{\ifleanmetaseen\else Lean: \global\leanmetaseentrue\fi\leanmetaproofpendinghandles}\else\refstepcounter{footnote}\footnotemark[\value{footnote}]\footnotetext[\value{footnote}]{\ifleanmetaseen\else Lean: \global\leanmetaseentrue\fi\leanmetaproofpendinghandles}\fi\global\let\leanmetaproofpendinghandles\@empty\fi}
\@ifundefined{newtheoremstyle}{}{%
  \newtheoremstyle{leanplain}
    {6pt}{6pt}{\itshape}{}{\bfseries}{.}{ }
    {\thmname{#1}\thmnumber{ #2}\leanmetaheadmark\thmnote{ (#3)}}
  \newtheoremstyle{leandefinition}
    {6pt}{6pt}{}{}{\bfseries}{.}{ }
    {\thmname{#1}\thmnumber{ #2}\leanmetaheadmark\thmnote{ (#3)}}
  \newtheoremstyle{leandef}
    {6pt}{6pt}{}{}{\bfseries}{.}{ }
    {\thmname{#1}\thmnumber{ #2}\leanmetaheadmark\thmnote{ (#3)}}
  \newtheoremstyle{leanremark}
    {6pt}{6pt}{}{}{\bfseries}{.}{ }
    {\thmname{#1}\thmnumber{ #2}\leanmetaheadmark\thmnote{ (#3)}}
}
\makeatother
\providecommand{\leanmeta}[1]{}
\renewcommand{\leanmeta}[1]{\ifhmode\unskip\footnote{\ifleanmetaseen\else Lean: \global\leanmetaseentrue\fi#1}\else\refstepcounter{footnote}\footnotemark[\value{footnote}]\footnotetext[\value{footnote}]{\ifleanmetaseen\else Lean: \global\leanmetaseentrue\fi#1}\fi}


==> paper_title_auto.tex <==
% Auto-generated by scripts/build_papers.py. Canonical manuscript title.
\providecommand{\PaperTitleAuto}{Thermodynamic Limits of Proof}

